HEJ 2.1: High-energy Resummation with Vector Bosons and Next-to-Leading Logarithms

We present version 2.1 of the High Energy Jets (HEJ) event generator for hadron colliders. HEJ is a Monte Carlo generator for processes at high energies with multiple well-separated jets in the final state. To achieve accurate predictions, conventional fixed-order perturbative QCD is supplemented with an all-order resummation of large high-energy logarithms. The new version 2.1 now supports processes with final-state leptons originating from a charged or neutral vector boson together with multiple jets, in addition to processes available in earlier versions. Furthermore, the all-order resummation is extended to include an additional gauge-invariant class of subdominant logarithmic corrections. HEJ 2.1 can be obtained from https://hej.hepforge.org.

==> Configurations.tex <==
\section{Emission of Quark-Antiquark Pairs}
\label{sec:qqbar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

